Revisiting Differentially Private Regression: Lessons From Learning Theory and their Consequences

Private regression has received attention from both database and security communities. Recent work by Fredrikson et al. (USENIX Security 2014) analyzed the functional mechanism (Zhang et al. VLDB 2012) for training linear regression models over medical data. Unfortunately, they found that model accuracy is already unacceptable with differential privacy when $\varepsilon = 5$. We address this issue, presenting an explicit connection between differential privacy and stable learning theory through which a substantially better privacy/utility tradeoff can be obtained. Perhaps more importantly, our theory reveals that the most basic mechanism in differential privacy, output perturbation, can be used to obtain a better tradeoff for all convex-Lipschitz-bounded learning tasks. Since output perturbation is simple to implement, it means that our approach is potentially widely applicable in practice. We go on to apply it on the same medical data as used by Fredrikson et al. Encouragingly, we achieve accurate models even for $\varepsilon = 0.1$. In the last part of this paper, we study the impact of our improved differentially private mechanisms on model inversion attacks, a privacy attack introduced by Fredrikson et al. We observe that the improved tradeoff makes the resulting differentially private model more susceptible to inversion attacks. We analyze this phenomenon formally.

==> comparison.tex <==
We note that the most relevant work is by Chaudhuri, Monteleoni and Sarwate~\cite{CMS11}
(see Section 4 for their analysis),
as well as Bassily, Smith and Thakurta~\cite{BST14}
(see Appendix F of their paper).

On one hand, to bound the generalization error,
\cite{CMS11} needs to assume the loss function to be smooth
(for their strongest bound, they need twice differentiability
with bounded derivatives).
Our work \emph{relaxes their technical requirements},
and we show that output perturbation can learn
\emph{any} convex-Lipschitz-bounded problem differentially privately.
Our bounds for generalization error match those obtained
in the recent work by Bassily et al.~\cite{BST14}.
However, \emph{our analysis is significantly simpler than both}.
On the other hand, the simplicity of our method does come at some cost.
Specifically, for general convex Lipschitz learning problems,
our bound for \emph{training error} is weaker than~\cite{BST14}.
(In terms of the dependence on $n$, ours is $1/n$, theirs is $1/n^2$).

Nevertheless, we believe that it is of importance to illustrate
the connection between the notion of stability in learning theory
and differential privacy. Perhaps more importantly, while the mechanisms
described in~\cite{BST14} give better training error,
their mechanisms are substantially more complicated.
More specifically, their mechanism uses a sophisticated sampling sub-procedure
that runs in time $O(n^3)$, where $n$ is the training set size.
For reasonably large data sets this can be prohibitive.
By contrast, we have demonstrated that output perturbation can already give
a good privacy/utility tradeoff for any convex-Lipschitz-bounded
learning problem. Given that output perturbation is possibly the one of
the easiest algorithms for differential privacy,
our method is potentially widely applicable in practice.
Indeed, in the rest of the paper, we will pursue the direction of
applying our method to training a linear regression model over some medical data.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> plot/Makefile <==
### Makefile --- 

TARGETS = out-fun-mse di-oracle-mse \
	out-fun-mi di-oracle-mi \
	bleed-compare mortality-compare stroke-compare\
	obj-di-oracle-mse

%: %.tex
	latexmk -g -pdf -silent $@ # generate pdf
	latexmk -c $@ # clean up regeneratable files

all: pdf

pdf: ${TARGETS}

clean:
	@echo cleaning up...
	rm -f *.fdb_latexmk *.ps *.dvi *.aux *.bbl *.blg *.brf *.cb *.cb2 \
		 *.idx *.ilg *.ind *.inx *.log *.mpx *.toc *.out *.pstex_t \
		 *.fig.bak  *.ps_e *~ *.tex.* *.thm *.fls


